In-context Learning with Retrieved Demonstrations for Language Models: A Survey

Language models, especially pre-trained large language models, have showcased remarkable abilities as few-shot in-context learners (ICL), adept at adapting to new tasks with just a few demonstrations in the input context. However, the model's ability to perform ICL is sensitive to the choice of the few-shot demonstrations. Instead of using a fixed set of demonstrations, one recent development is to retrieve demonstrations tailored to each input query. The implementation of demonstration retrieval is relatively straightforward, leveraging existing databases and retrieval systems. This not only improves the efficiency and scalability of the learning process but also has been shown to reduce biases inherent in manual example selection. In light of the encouraging results and growing research in ICL with retrieved demonstrations, we conduct an extensive review of studies in this area. In this survey, we discuss and compare different design choices for retrieval models, retrieval training procedures, and inference algorithms.

==> 05_old_application.tex <==
\section{Applications} \label{sec:application}

The effectiveness of retrieval-based ICL have been showed in four types of tasks. 1). Natural Language Understanding Tasks. These  include sentiment analysis (SA): SST-5~\citep{socher2013recursive},SST-2~\citep{socher2013recursive}, Yelp~\citep{zhang2015character}, Sent140~\citep{go2009twitter};
paraphrase detection (PD): MRPC~\citep{dolan2004unsupervised}, PAWS~\citep{paws2019naacl};
reading comprehension (RC): SQuAD~\citep{rajpurkar2016squad}, MultiRC~\citep{MultiRC2018}, BoolQ~\citep{clark2019boolq}, OBQA~\citep{}, natural language inference (NLI): MNLI ~\citep{williams2018broad}, QNLI~\citep{wang2018glue}, SNLI~\citep{}, RTE~\citep{}. 
The retrieval-based ICL shows noticeable improvements on SA and NLI tasks~\citep{liu2022makes,ye2023compositional}. 

2). Reasoning tasks. These include mathematical reasoning~\citep{cobbe2021gsm8k}, commonsense reasoning (CSR): CMSQA~\citep{talmor2019commonsenseqa}, HellaSwag~\citep{zellers2019hellaswag}, PiQA~\citep{Bisk2020}, COPA~\citep{roemmele2011choice}; and ethical Reasoning~\citep{jiang2021can}.  
Coreference Resolution (CR),  Winogrande~\citep{levesque2012winograd}. Such tasks are usually accompany by CoT, but ~\citet{zhang2022automatic} founds that CoT does not help that much for the commonsense reasoning task. Many works have shown that retrieval based methods are worse than random demonstrations on commonsense reasoning tasks (e.g. CMSQA). Simple similarity based retrieval method does not show significant improvement on mathematical reasoning task, and ~\citet{zhang2022automatic} shows that diversity is important for mathematical reasoning tasks. The iterative retrieval retrieval strategy shows the most significant improvement on mathematical reasoning tasks~\cite{scarlatos2023reticl}. 


3). Knowledge Based QA. In such a task, the question is given and it requires external knowledge to answer the question: WebQs~\citep{berant2013semantic}, NQ~\citep{kwiatkowski2019natural}, TriviaQA~\citep{joshi2017triviaqa}, Webquestion~\citep{berant2013semantic}, ARC-e/c~\citep{clark2018think}.
To tackle such tasks, the state-of-the-art systems usually retrieve relevant passages that might contain the answer to the question, and then feed such passages and questions together to a language model to generate the answer. \citet{ye2023compositional} shows that BM25 achieve 10+\% improvement on open-domain QA\citep{berant2013semantic}
The last one is Text Generation. This includes code generation (CodeGen): GeoQuery~\citep{zelle1996learning}, NL2Bash~\citep{lin2018nl2bash}, semantic parsing (SP): Break~\citep{wolfson2020break}, MTOP~\citep{li2021mtop}, SMCalFlow\citep{andreas2020task};
text-to-SQL~\citep{shi2022xricl}, Table-to-text(Table2Text) generation~\citep{parikh2020totto}; 
Data-to-Text (D2T): CommonGen~\citep{}, DART~\citep{nan2021dart}, E2E NLG~\citep{duvsek2019semantic}. 
~\cite{rubin2021learning} shows that the retrieved demonstrations significantly outperform random demonstrations. (e.g. BM25 is 25+\% better than random, and EPR is 30\% better than random).  

Apart from different types of tasks, some work shows that when there is a low-resource of training data, retrieval-augmented is even better than fine-tuning a model on the low-resource data. Also, retrieving from a high-resource domain can benefit a low-resource domain, for example cross-lingual. 

% \mk{I suggested that we look for papers that are \textbf{not} specifically focused on demonstration retrieval, but they try to solve some task X and they find that adding demonstration retrieval helps improve their task. For example, we may find a paper that tries to solve molecule generation with LLMs, and they mention that demonstration retrieval helped them.}

==> old_text.tex <==

\paragraph{Few-shot In-context Learning}
% In-context learning is first introduced in GPT, given a description of the tasks with few examplars (input-output), language models can generalize to unseen tasks. However, many work shows that In-context learning performance varies by many factors, such as the ordering of the demonstrations~\cite{kumar2021reordering}, the distribution of the demonstrations~\cite{}.
% \citet{} found that a prompt with lower perplexity is better than ones with higher perplexity.
% \citet{zhao2021calibrate} found that LLMs suffer from majority label bias, recency bias, and common token bias. \citet{arora2022ask} found that the open-ended question answer format is more effective than restrict output format.  
% In the beginning, the prompts are usually written by human, which require many engineering and can be sub-optimal.  
% Thus, many follow-up work introduce automatic methods to generate prompts~\cite{}.  
% Improving few shot in-context learning~\cite{nie2022improving}.
% More recently, Chain-of-thought prompting~\cite{wei2022chain}, generating a series of intermediate reasoning steps (input-explanation-output), enhances the reasoning performance of LLMs on complex tasks ~\cite{suzgun2022challenging}. 
% \citet{wang2022towards} found that even though with invalid reasoning steps, LLMs can still achieve good performance on reasoning tasks. 
% \citet{fu2022complexity} shows that prompt with higher  reasoning complexity achieves better performance on math word reasoning tasks. 
% There are also research to study how in-context learning works. 
% \citet{xie2021explanation} shows that ICL is implicit Bayesian inference.
% \citet{madaan2022text} show that a symbiotic relationship between text and patterns explains the success of few-shot prompting.
% \citet{dai2022can} proves that ICL behaves similarly to explicit finetuning at the prediction level, the representation level, and the attention behavior level.


Few-shot in-context learning (ICL) is a technique that allows language models, such as GPT-3~\citep{brown2020language} and PaLM~\citep{chowdhery2022palm}, to generalize to new tasks based on a small number of examples. 
ICL offers several advantages over the traditional training approach of language models, which involves pre-training followed by fine-tuning. One key benefit is that fine-tuning may not always be feasible due to restricted access to the LLM or inadequate computational resources~\citep{brown2020language}.
Additionally, ICL avoids the issues commonly associated with fine-tuning, such as overfitting~or~shocks~\citep{ying2019overview,kazemi2023understanding}, as it does not modify the model's parameters, allowing it to remain general.
However, the effectiveness of ICL varies depending on various factors, such as the order of the demonstrations~\citep{kumar2021reordering}, the distribution of the demonstrations~\citep{min2022rethinking}, and the complexity and quality of the prompts themselves~\citep{zhao2021calibrate,arora2022ask}. Some research has shown that lower perplexity prompts~\citep{gonen2022demystifying} and open-ended question-answer formats~\citep{arora2022ask} tend to lead to better performance, while others have found that intermediate reasoning steps~\citep{wei2022chain} and higher complexity prompts~\citep{fu2022complexity} can also improve results on certain tasks~\citep{suzgun2022challenging,wang2022towards}.
In an effort to understand how ICT works, studies have suggested that ICL may involve implicit Bayesian inference~\cite{xie2021explanation} and a symbiotic relationship between text and patterns~\cite{madaan2022text}, and can behave similarly to explicit fine-tuning~\cite{dai2022can}.
Our work focus on the effect of demonstrations for ICL with large language models. 

% \subsection{Retrieval Augmented Large Language Models}
\paragraph{Retrieval Augmented Demonstrations}


\yl{Is this paragraph in essence a detailed description of Table 1? Could we move it to the start of Section 3?}

\yl{Table 1 is a very good taxonomy of retrieved few-shots learning, could actually be our main contribution as a survey paper. I would suggest giving a high-level overview of this table, walk readers through the columns and explain why do we classify the works in those axes? For each column/axis, explain what is the key problem/challenge, how does current work solves it.}

% Retrievers have been used to enhance language models through inputs, attention, memory, and output augmentation. Here, we mainly discuss the input augmentation. 
% Different ways to augment the inputs have been studied, including retrieving knowledge from Wikipedia~\cite{izacard2022few} or from internet~\cite{lazaridou2022internet}, retrieving explicit demonstrations~\cite{Nie2022CrossLingualRA} and implicit demonstrations~\cite{chen2022decoupling} for few-shot in-context learning, where the demonstrations are from the training datasets of the target tasks. 
% ~\citet{liu2022makes} found that semantically-close demonstrations are more effective than random demonstrations.
% % Most of the work uses k-Nearest Neighbour method based on semantic representations or BM25~\cite{robertson2009probabilistic} to select the demonstrations. 
% ~\citet{rubin2021learning} train a retriever based on the signal from language models. 
% ~\citet{ram2023context} uses a cross-attention reranker to re-rank the documents retrieved by BM25.
% ~\citet{madaan2022memory,dalvi2022towards} use human feedback and dynamically add the demonstrations to a retriever bank. 
% Our study has uncovered more applications for retrieval-based demonstrations in one-shot and few-shot inference, spanning from general language models to instruction-finetuned ones, as well as simple and advanced prompts, such as Chain-of-Thought.

As summarized in Table~\ref{tab:related_work},
several previous works have explored retrieval techniques for identifying more informative demonstrations to boost in-context learning.
KATE~\citep{liu2022makes} discovers that semantically closer demonstrations outperform random ones for GPT-3 in-context learning. They employ language models trained on tasks like natural language inference and sentence textual similarity as semantic representations and utilize the kNN algorithm to search for demonstrations.
EPR~\citep{rubin2021learning} develops a retriever based on language model signals to find superior demonstrations compared to off-the-shelf retrievers. Instead of using a separate retriever for each task, UPRISE~\citep{cheng2023uprise} merges multiple training datasets into a retrieval corpus and trains a universal retriever for cross-domain tasks.
PARC~\citep{Nie2022CrossLingualRA} employs a multilingual retrieval strategy to find demonstrations from high-resource tasks, thereby enhancing the performance of low-resource domain tasks. CEIL~\citep{ye2023compositional}, instead of retrieving few-shot demonstrations independently, introduces an iterative retrieval method to identify both diverse and similar few-shot examples.
While the aforementioned methods retrieve demonstrations from training data, \citep{madaan2022memory,dalvi2022towards} incorporate human feedback to create demonstrations and maintain a dynamic retrieval corpus. Z-ICL~\citep{lyu2022z} generates pseudo demonstrations to enhance zero-shot in-context performance.
In contrast to the methods that retrieve explicit demonstrations, RETROPROMPT~\citep{chen2022decoupling} transforms explicit demonstrations into implicit neural demonstrations represented by vectors. Rather than using a retriever, ~\citep{ram2023context} applies a cross-attention reranker to re-rank documents retrieved by BM25.

==> pros_cons.tex <==
% \ml{Discuss Table 1 during the meeting}


% Retrieval inference latency depends on the efficiency of the retriever and also the size of the retrieval corpus. 

% - BM25:sparse retriever, is it faster than dense retriever?

% - Dense Retriever: 

% - ColBERT 

% - Reranker 

% How do we put them in the table? 

% LLM inference latency depends on how large the LLM is and also adding more shots will increase the input length that also makes the inference slow. again, how to categorize them?

% Cost of Training data for retriever. 

% Depends on how to obtain the retriever training data. 

% - does it use LLM to get the signal? Xin, I remember there are some paper that does not use LLM?

% - Does it use a large LLM or a small LLM? 


% Annotation of Retrieval corpus. 

% - does the pipeline depends on human annotated data? 

% - use a small portion? 

% - does not depends on any human annotated data? 


% Universal Retriever v.s. in-domain retriever 








\begin{table*}[!htbp]
    \centering
    \small
    \resizebox{0.99\linewidth}{!}{
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{@{}p{0.2\linewidth}p{0.25\linewidth}p{0.40\linewidth}@{}}
        \toprule
        \textbf{Retriever} & \textbf{Efficiency}  & \textbf{Performance} \\
        \toprule
    BM25 & no training, indexing requires less memory, one method for all tasks & better than random \\
    \midrule
    Sentence Embedding Similarity & requires a pretrained model, indexing requires large memory, one method for all tasks &  better than random \\
    \midrule
    Pretrained Dual Encoder & requires a pretrained neural retriever, indexing requires large memory, one method for all tasks &  better than random and Sentence Embedding Similarity \\
    \midrule
    Fine-tuned Demonstrations Retriever & require training, indexing require large memory, single model for one task. & better than random and the methods without training\\ 
   
    \bottomrule
    \end{tabular}
    }
    \caption{We compare the pros and cons of different types of retrievers. 
    }
    \label{tab:pros_cons} 
\end{table*}

==> table_summary.tex <==
\begin{table*}[!htbp]
    \centering
    \small
    \resizebox{0.99\linewidth}{!}{
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{@{}p{0.1\linewidth}p{0.1\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}@{}}
        \toprule
        \textbf{Paper} & \textbf{LLMs}  & \textbf{Retrieval Method}  & \textbf{Retrieval Corpus} & \textbf{Evaluation Tasks}& \textbf{ \# of Shots in Prompts} & CoT\\
        \toprule
    KATE~\citeyear{liu2022makes} & GPT-3 & RoBERTa+kNN & In-Domain TD & SA, Tab2Text, QA & Few-shots & No \\
    \midrule
    EPR~\citeyear{rubin2021learning} & GPT-J, CODEX, GTP-3 & SBERT, BM25, FT Retriever & In-Domain TD & SP& One-shot, Few-shots& No \\
    \midrule
    CEIL~\citeyear{ye2023compositional}& GPT-NEO, GPT2-XL, CODEX & BM25, BERT, FT Retriever & In-Domain TD & SA, PD, NLI, CSR, QA, CodeG, and SP & Few shots & No\\
    \midrule
    UP
    RISE~\citeyear{cheng2023uprise} & GPT-Neo, BLOOM, OPT, GPT-3 & FT Retriever & Cross Tasks TD & RC, QA, NLI, SA, CSR, CR, PD & Few shots& No\\
    \midrule
    Dr.ICL~\citeyear{luo2023dr} & PaLM, Flan-PaLM & BM25, GTR, FT Retriever &  In-Domain TD & QA, NLI, MathR, BC & One-shot, Few-shots & Yes \\
    \midrule
    LLM-R~\citeyear{wang2023learning} & LLaMA-7B & FT Retriever and Reranker  & Multi TD  & QA, CSR, CR, Paraphrase, RC,SA, D2T, Summarization, NLI & Few shots & No\\
    \midrule
    Z-ICL~\citeyear{lyu2022z} & GPT-J, GPT-NeoX, GPT-3 & SimCSE & Mixed text corpus with no training labels & SA, sentence classification tasks & few-shots & No\\
    \midrule
    Mem
    Prompt~\citeyear{madaan2022memory}& GPT-3 & Fine-tuned Generative Retriever & Human-feedback and In-Domain TD & Lexical Relations, Word Scrambling, Ethical Reasoning & few-shots & No\\
    \midrule
    Teach
    Me~\citeyear{dalvi2022towards} & T5-11B & BM25 & Human Feedback In-Domain TD&  QA & Few-shots & No\\
    \midrule
    UDR~\citeyear{li2023unified} & GPT-J, GPT-Neo, CODEX, GPT-3 & Fine-tuned Unified Retriever & Multi TD & 13 Tasks families & Few-shots & No\\
    \midrule
    IC-DST~\citeyear{hu2022context} & GPT-3 & Fine-tuned SBERT Retriever & In-domain TD & DST-to-SQL & Few-shots & No \\
    \midrule
    Mot~\citeyear{li2023mot} & ChatGPT & SBERT for clustering and filtering, LLM as retriever & LLM Generated CoT for TD & MathR, NLI, CSR, QA  & Few-shots, & Yes\\
    \midrule 
    vote-k~\citeyear{hongjin2022selective} & GPT-Neo,GPT-J,GPT-3, CODEX & SBERT & Selected subsets of TD, labelled &SA, NLI, QA, Summarization, CSR, RC &  Few-shots & No \\
    \midrule 
    XRICL~\citeyear{shi2022xricl} & CODEX & Fine-tuned Retriever, reranker & cross-lingual, in-domain TD & Text-to-SQL & Few-shots & No \\
    \midrule 
    Auto-CoT~\citeyear{zhang2022automatic} & GPT-3 & Clustering with SBERT, one-demo per cluster & LLM Generated CoT for TD  & MathR, QA & Few-shots & Yes \\
    \midrule
    DSP~\citeyear{khattab2022demonstrate} & GPT-3 & ColBERTv2 & In Domain TD & QA & Few-shots & No \\
    \midrule
    PARC~\citeyear{Nie2022CrossLingualRA} & mBERT & Multilingual SBERT & Cross-lingual, in-domain TD & SA, TopicC, NLI & Few-shots  & No\\
    \midrule
    Cover-LS~\citeyear{levy2022diverse}- & CODEX, T5-large & Custom diversity optimizing algorithm  &  In Domain & SP & Few-shots & No \\
    \midrule 
    RetICL~\citeyear{scarlatos2023reticl} & CODEX & SBERT & In Domain  & MathR & Few-shots & Yes \\
    \midrule
    Prompt
    PG~\citeyear{lu2022dynamic} & GPT-3 & - &  - &  TQA  & Few-shots & Yes \\
    \midrule 
    Ambig-ICL~\citeyear{gao2023ambiguity} & Flan-PaLM & fine-tuned mT5, plus a filtering algorithm based on LLM feedback & In Domain & TC, SA & Few-shots & No\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison with Related Work. TD: training data, QA: question answering, RC: reading comprehension, NLI: natural language inference, SA: sentiment analysis, CSR: commonsense reasoning, CR: Coreference Resolution, MathR: mathematical reasoning, PD: paraphrase detection, SP: semantic parsing, CodeG: code generation, Tab2Text: Table to Text generation, DST: Dialogue State Tracking, TQA: Table Question Answering
    }
    \label{tab:related_work} 
\end{table*}


